Examining Common Paradigms in Multi-Task Learning

While multi-task learning (MTL) has gained significant attention in recent years, its underlying mechanisms remain poorly understood. Recent methods did not yield consistent performance improvements over single task learning (STL) baselines, underscoring the importance of gaining more profound insights about challenges specific to MTL. In our study, we investigate paradigms in MTL in the context of STL: First, the impact of the choice of optimizer has only been mildly investigated in MTL. We show the pivotal role of common STL tools such as the Adam optimizer in MTL empirically in various experiments. To further investigate Adam's effectiveness, we theoretical derive a partial loss-scale invariance under mild assumptions. Second, the notion of gradient conflicts has often been phrased as a specific problem in MTL. We delve into the role of gradient conflicts in MTL and compare it to STL. For angular gradient alignment we find no evidence that this is a unique problem in MTL. We emphasize differences in gradient magnitude as the main distinguishing factor. Overall, we find surprising similarities between STL and MTL suggesting to consider methods from both fields in a broader context.

==> chapters/03c_exps+res_gen2data.tex <==
\subsection{Robustness of multi-task representations on corrupted data}
\label{sec:exp_ood}

In the last part of our analysis, we investigate whether features learned for multiple tasks generalize better to corrupted data compared to those learned for single tasks only.


\textit{Motivation:} 
In his seminal paper, Caruana gives preliminary evidence that MTL provides stronger features and avoids spurious correlations (referred to better \emph{attribute selection})~\cite{caruana1997multitask}. More recently, spurious correlations have often been directly connected with robustness \cite{geirhos2020shortcut, ilyas2019adversarial}. 
Results from current literature on the robustness of MTL features are mixed. While MTL is stated to increase the adversarial- and noise-robustness over STL\cite{klingner2020improved,mao2020multitask,yeo2021robustness}, others argue features selected by MTL could be more likely to be non-causal and, therefore, less robust~\cite{hu2022improving,beery2018recognition}.
Here, we further examine the paradigm whether MTL features lead to better robustness. 
We would like to nuance that we do not consider the transferability of representations, e.g., to new tasks, but solely focus on the claim that the MTL trained features are more robust w.r.t.\ different inputs. 


\textit{Approach:} 
In our experiment, we treat the common corruptions~\cite{hendrycks_robustness_2019} as downstream task and compare the performance after fine-tuning the heads on corrupted data while freezing the pre-trained STL/MTL backbone.
While this differs from the typical OOD setup, here, it allows us to explore whether MTL or STL yield more robust representations for corrupted data.

We select models trained on clean data with the best performing hyperparameter configuration from previous experiments and fine-tune their heads on corrupted data.
Following this, we compare the test performance of models trained in the multi-task setup to those that were learned for a single-task only.
We use the perturbation modes proposed by Hendrycks et al.~\cite{hendrycks_robustness_2019} which include different variants of noise, blur, and weather conditions and apply five levels of severity.
We randomly select corruption and severity level for each data sample during fine-tuning and create a corrupted versions of the test data w.r.t. all proposed corruptions and perturbation levels. 


To quantify the robustness of single- and multi-task models, we first compute the individual task metrics $M$ (e.g., mIoU) per task $t$ for a STL and MTL network. Next, we compute the relative performance when each model is faced with corrupted data. Lastly, we calculate the difference of relative performances of the MTL compared to the STL model. 
In detail, over all corruption modes $C$ and levels of severity $S$ we have 
\begin{align}
    \label{eq:ood_eval}
    \delta_t &= \frac{1}{|C|\cdot |S|}\sum_{c\in C}\sum_{s\in S}(-1)^{p(t)}\delta_{t,c,s} \\ \nonumber
    & \text{with} \quad \delta_{t,c,s} = \frac{M^{MTL, corrupted}_{t,c,s}}{M^{MTL, clean}_{t}} - \frac{M^{STL, corrupted}_{t,c,s}}{M^{STL, clean}_{t}}
\end{align}
where $p(t)=1$ if a higher value on task $t$ corresponds to better performance and $p(t)=0$ otherwise.
This metric yields $\delta_t<0$ if the MTL model was able to handle data corruption better. If the STL model is less impacted, we get $\delta_t>0$.

\input{figures/ood_cityscape_deeplab}
\input{tables/ood_cs_deeplab}
\textit{Results:} \Cref{fig:ood_cityscapes_deeplab} shows $\delta_t$  for different corruption types for a DeepLabV3 with EW on Cityscapes averaged over five corruption levels and three seeds.
On the semantic segmentation tasks, the STL models show a slightly lower decrease in performance on the corrupted data than MTL ($\delta_t>0$ more often; shaded in red), indicating that the features learned for these respective tasks can better generalize to corrupted data.
In contrast, the MTL model shows significant better relative performance on the depth task ($\delta_t<0$  more often; shaded green). 
Comparing these observations to other dataset+network combinations (\cref{fig:ood_more}), we find a strong robustness of MTL features for both setups of CityScape+SegNet and NYUv2+DeepLabV3 over all tasks. However, evaluation on NYUv2+SegNet resulted on average in better performance on STL features, especially for the depth task.
%
Furthermore, we see little evidence for general higher robustness against certain types of corruption (e.g., higher robustness against weather conditions) for either MTL or STL across all setups.



The results of other MTO methods (\cref{tab:ood_cityscapes_deeplab,tab:ood_cityscapes,tab:ood_nyu_segnet_deeplab}) indicate that it depends less on the used method but more on the choice of dataset and network architecture whether some tasks would benefit from MTL for learning more robust features. Averaged absolute scores can be found in \cref{tab:ood_cityscapes_abs,tab:ood_nyu_abs}.





\textit{Conclusion:}
Our experiments show that MTL \textit{can} result in learning more robust features, either for a subset of tasks or even all. However, we could not observe a uniform pattern whether certain tasks consistently benefit from MTL.
Instead, it depends on the task, the type of corruption, the network, and the dataset whether MTL or STL is superior towards corrupted data. Whether there is a general pattern, we leave to further research. 
%
We further cannot fully confirm the outcome of \cite{klingner2020improved} as only two of our setups have indicated that the segmentation task can be more robust in the MTL setting.
%
Controversial to the claim of \cite{mao2020multitask}, our evaluation shows that none of the MTL approaches, even IMTL, PCGrad or CAGrad which adjust the gradients, yields consistent values of $\delta_t<0$ which would have shown an advantage of certain MTO methods over STL. 




==> figures/cagrad_toytask_full_jpg.tex <==
\begin{figure}[ht]
\centering
\scriptsize
\newcommand{\gcs}{\hspace{4pt}}
\begin{tabular}{cc@{\gcs}ccccccc}
    && \multicolumn{7}{c}{GD} \\
    \cmidrule(){3-9}
    && 1.0 & 0.5 & 0.1 & 0.05 & 0.01 & 0.005 & 0.001 \\
    \rotatebox{90}{\hspace{10pt} EW} && 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_sgd_1.0.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_sgd_0.5.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_sgd_0.1.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_sgd_0.05.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_sgd_0.01.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_sgd_0.005.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_sgd_0.001.jpg}\\
    \rotatebox{90}{\hspace{1pt} PCGrad} && 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_sgd_1.0.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_sgd_0.5.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_sgd_0.1.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_sgd_0.05.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_sgd_0.01.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_sgd_0.005.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_sgd_0.001.jpg}\\
    \rotatebox{90}{\hspace{1pt} CAGrad} && 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_sgd_1.0.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_sgd_0.5.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_sgd_0.1.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_sgd_0.05.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_sgd_0.01.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_sgd_0.005.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_sgd_0.001.jpg}\\
    \midrule
    && \multicolumn{7}{c}{Adam} \\
    \cmidrule(){3-9}
    && 1.0 & 0.5 & 0.1 & 0.05 & 0.01 & 0.005 & 0.001 \\
    \rotatebox{90}{\hspace{10pt} EW} && 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_adam_1.0.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_adam_0.5.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_adam_0.1.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_adam_0.05.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_adam_0.01.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_adam_0.005.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/ew_adam_0.001.jpg}\\
    \rotatebox{90}{\hspace{1pt} PCGrad} && 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_adam_1.0.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_adam_0.5.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_adam_0.1.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_adam_0.05.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_adam_0.01.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_adam_0.005.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/pcgrad_adam_0.001.jpg}\\
    \rotatebox{90}{\hspace{1pt} CAGrad} && 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_adam_1.0.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_adam_0.5.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_adam_0.1.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_adam_0.05.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_adam_0.01.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_adam_0.005.jpg} & 
    \includegraphics[trim = 15mm 2mm 25mm 0mm, clip, width=0.12\textwidth]{imgs/toytask_cagrad_jpg/cagrad_adam_0.001.jpg}\\
\end{tabular}
\caption{
Extension of \Cref{fig:cagrad_toytask} with additional learning rates. 
We show the optimization trajectories for three different seeds (black dots).
The Optimization trajectories are colored from {\color{red}red} to {\color{Dandelion}yellow} for 100k iteration steps.
The global optimum is depicted as asterix ($\ast $), the Pareto front is highlighted in gray.
We note the importance of a good selection of learning rate even for simple toy examples.
Moreover, using Adam yields overall faster convergence to the global optimum.
We use the original implementation which can be found under \url{https://github.com/Cranial-XIX/CAGrad}
.} 
\label{fig:cagrad_toytask_extended}
\end{figure}


==> tables/adam_EW_nyu_cancel.tex <==
\begin{table*}[h]
\centering
\small
\caption[Comparison of Equal Weighting with different scales using the Adam optimizer for NYUv2.]{Comparison of Equal Weighting with different scales using the Adam optimizer for NYUv2. We show results for EW with $w=1$ and $w=10$ with a single random seed. 
}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrrrrrrrr}
%\multirow{7}{*}{SegNet}
\toprule
               \multirow{3}{*}{Method} & \multicolumn{2}{c}{Segmentation $\uparrow$} & \multicolumn{2}{c}{Depth $\downarrow$} & \multicolumn{5}{c}{Surface Normal} & \multirow{3}{*}{$\Delta_m\%\downarrow$} \\
                       &  & & & & \multicolumn{2}{c}{Angle Distance $\downarrow$} & \multicolumn{3}{c}{Within $t^{\circ}$ $\uparrow$} &\\
                    % &   &  &  & & &  
                     &        mIoU & Pix Acc &        Abs Err & Rel Err &           Mean & Median &           11.25 &    22.5 & \multicolumn{2}{l}{30} \\
\midrule 
EW $w=1$ &         $0.412$ & $0.665$ &        $0.516$ & $0.210$ &         $28.2$ & $23.2$ &         $0.231$ & $0.487$ & $0.618$ &         $4.9$ \\
EW $w=10$ &         $0.406$ & $0.665$ &        $0.521$ & $0.213$ &         $28.1$ & $23.1$ &         $0.232$ & $0.488$ & $0.620$ &         $4.9$ \\
\bottomrule
\end{tabular}}
\label{tab:nyuv2_EW_adam}
\end{table*}

==> tables/adam_parameter_values_toy_experiment.tex <==
\begin{table}[h]
\centering
\small
\caption[Learned network parameter values in the last training epoch using the Adam optimizer with equal and non-uniform task weights.]{Learned network parameter values in the last training epoch using the Adam optimizer with equal and non-uniform task weights. The parameter values are equal for the two EW scenarios, but differ using non-uniform task weights.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|llllll}
\hline
 & \multicolumn{6}{l}{Parameters} \\ \hline
 & backbone weight & backbone bias & head 1 weight & head 1 bias & head 2 weight & head 2 bias \\ \hline
 EW $w=1$ & [0.7458,-0.2706] & [-0.6616, -0.4992] & [0.1554, 0.1600] & [-0.2587] & [0.1308, -0.0818] & [0.4273] \\
EW $w=10$ & [0.7458,-0.2706] & [-0.6616, -0.4992] & [0.1554, 0.1600] & [-0.2587] & [0.1308, -0.0818] & [0.4273] \\
Non-uniform & [0.9135,-0.2706] & [-0.4925, -0.4992] & [0.2105, 0.1600] & [-0.2587] & [0.0757, -0.0818] & [0.4273] \\
\end{tabular}}
\label{tab:adam_toy}
\end{table}

==> tables/ood_cs_deeplab.tex <==
\begin{table*}[tb]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{4pt}  % default: 6pt
    \newcommand{\gcs}{\hspace{12pt}}
    \newcommand{\customdashline}{\cdashline{2-10}\noalign{\vskip 0.5ex}}
    \caption{
        \textbf{Out-Of Distribution transfer on corrupted Cityscapes~\cite{cordts_cityscapes_2016} for different MTO methods on DeepLabV3.}
        We report difference between relative performance decrease for STL and MTL averaged over all modes of corruption and all levels of severity (\cref{eq:ood_eval}) as well as over runs for three seeds.
        A value lower than zero indicates a better generalization capability of the MTL backbone and vice versa.
    }
    \begin{tabular}{llc@{\gcs}ccc@{\gcs}ccc@{\gcs}c}
    \toprule
        &&& \multicolumn{2}{c}{Sem.Seg.} && \multicolumn{2}{c}{Depth}  && Mean\\
        \cmidrule(){4-5}\cmidrule(){7-8}\cmidrule(){10-10}
        Network & MTO  && $\delta_{\text{mIoU}}$  & $\delta_{\text{pixAcc}}$   && $\delta_{\text{AbsErr}}$  & $\delta_{\text{RelErr}}$  &&  \\
        \midrule
        DeepLabV3 & EW && 0.0087 & 0.0017 && -0.0108 & -0.1826 && -0.0457 \\
        \customdashline
        ~ & UW && 0.0110 & 0.0018 && 0.1179 & 0.0861 && 0.0542 \\
        ~ & RLW && 0.0263 & 0.0084 && -0.0809 & -0.3595 && -0.1015 \\
        ~ & IMTL && 0.0172 & 0.0041 && 0.1747 & 0.0857 && 0.0704 \\
        ~ & PCGrad && 0.0090 & 0.0019 && 0.0394 & -0.2240 && -0.0434 \\
        ~ & CAGrad && 0.0224 & 0.0067 && 0.0898 & -0.2841 && -0.0413 \\
    \bottomrule
    \end{tabular}
    \label{tab:ood_cityscapes_deeplab}
\end{table*}

==> tables/ood_nyu.tex <==

\begin{table}[t]
    \centering
    \tiny
    \setlength{\tabcolsep}{1pt}  % default: 6pt
    \newcommand{\gcs}{\hspace{2pt}}
    \newcommand{\customdashline}{\cdashline{1-9}\noalign{\vskip 0.5ex}}
    \caption{
        \textbf{Out-Of Distribution transfer on corrupted NYUv2~\cite{silberman_nyuv2_2012} for different networks and MTO methods.}
        We report difference between relative performance decrease for STL and MTL averaged over all modes of corruption and severity (cf. \Cref{eq:ood_eval}). Mean of three runs is reported.
    }
    \begin{tabular}{lc@{\gcs}cccccc@{\gcs}c}
    \toprule
        && \multicolumn{2}{c}{Sem.Seg.} && \multicolumn{2}{c}{Depth} \\
        \cmidrule(){3-4}\cmidrule(){6-7}
         MTO  && $\delta_{\text{mIoU}}$  & $\delta_{\text{pixAcc}}$   && $\delta_{\text{AbsErr}}$  & $\delta_{\text{RelErr}}$ \\
        \midrule
        EW & ~ & 0.0139 & 0.0134 & ~ & 0.0715 & 0.0922  & ~ \\ 
        \customdashline
        UW & ~ & 0.0166 & 0.0149 & ~ & 0.1146 & 0.1225 & ~ \\ 
        RLW & ~ & 0.0174 & 0.0223 & ~ & -0.0062 & 0.0281 & ~ \\ 
        IMTL & ~ &  0.0073 & 0.0123 & ~ & 0.1108 & 0.1247 & ~ \\ 
        PCGrad & ~ & 0.0186 & 0.0174 & ~ & 0.0720 & 0.0817 & ~ \\ 
        CAGrad & ~ & 0.0061 & 0.0116 & ~ & 0.1172 & 0.1428 & ~ \\
        \midrule
        && \multicolumn{5}{c}{Normal} && Mean\\    
        \cmidrule(){3-7}\cmidrule(){9-9}
        && $\delta_{\text{Mean}}$  & $\delta_{\text{Median}}$  & $\delta_{<11.25}$ & $\delta_{<22.5}$ & $\delta_{<30.0}$ &  \\
        \midrule
        EW & ~ & -0.0836 & -0.1492 & 0.0293 & 0.0168 & 0.0116 && 0.0018 \\ 
        \customdashline
        UW & ~ & -0.0564 & -0.0984 & 0.0313 & 0.0207 & 0.0164 && 0.0203 \\ 
        RLW & ~ & -0.1048 & -0.1857 & 0.0229 & 0.0089 & 0.0055 && -0.0213 \\ 
        IMTL & ~ & -0.0186 & -0.0390 & 0.0361 & 0.0274 & 0.0228 && 0.0315 \\ 
        PCGrad & ~ & -0.0702 & -0.1271 & 0.0264 & 0.0158 & 0.0121 && 0.0052 \\ 
        CAGrad & ~ & -0.0082 & -0.0202 & 0.0465 & 0.0286 & 0.0223 && 0.0385 \\ 
    \bottomrule
    \end{tabular}
    \label{tab:ood_nyu}
\end{table}


==> tables/res_cs_deeplab.tex <==
\begin{table}[!ht]
    \centering
    \tiny
    % \setlength{\tabcolsep}{6pt}  % default: 6pt
    \newcommand{\gcs}{\hspace{12pt}}
    \newcommand{\customdashline}{\noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}}
    \caption{
    \textbf{Results for different MTO methods and optimizers on Cityscapes~\cite{cordts_cityscapes_2016} using DeepLabV3+~\cite{chen_deeplabv3_2018}.}
    The best score per metric is highlighted \textbf{for each MTO method} as well as \underline{over all methods and optimizers}.
    Adam is Pareto dominant over SGD+mom in a direct paiwise comparison across all MTO methods.
    }
    \begin{tabular}{cccc@{\gcs}ccc@{\gcs}ccc@{\gcs}c}
    \toprule    
        &&&& \multicolumn{2}{c}{Sem.Seg.} && \multicolumn{2}{c}{Depth}\\
        \cmidrule(r){5-6} \cmidrule(r){8-9}
        MTO & Optimizer & lr && mIoU $\uparrow$ & pixAcc $\uparrow$  && AbsErr $\downarrow$  & RelErr $\downarrow$ && DeltaM $\downarrow$\\
    \midrule
        %STL & adam & && 0.7380 & 0.9326 && 0.0121 & 40.03 \\
        STL & adam & && 0.7203 & 0.9253 && 0.0132 & 47.37 \\
    \midrule
        EW & adam & 0.001 &&     \textbf{\underline{0.7247}} & \textbf{0.9268} && \textbf{0.0128} & \textbf{47.73}  && \textbf{-0.80} \std{0.69}\\ 
        EW & signSGD & 0.0005  && 0.7188 & 0.9249 && 0.0134 & 52.47 && 3.07 \std{2.70}\\
        EW & sgd & 0.05 &&       0.7100 & 0.9217 && 0.0174 & 120.34 && 46.88 \std{2.02}\\ \customdashline
        UW & adam & 0.001 &&     \textbf{0.7224} & \textbf{0.9259} && \textbf{0.0122} & \textbf{\underline{44.37}} && \textbf{\underline{-3.65}}\std{0.61}\\ 
        UW & signSGD & 0.001  && 0.7172 & 0.9244 && 0.0127 & 48.31 && -0.35 \std{2.23}\\
        UW & sgd & 0.005 & &     0.7003 & 0.9187 && 0.0171 & 116.09 && 44.47 \std{1.91}\\ \customdashline
        RLW & adam & 0.001 &&    \textbf{0.7230} & \textbf{0.9263} && \textbf{0.0133} & \textbf{47.76} && \textbf{0.26} \std{1.08} \\ 
        RLW & signSGD & 0.001  && 0.7185 & 0.9244 && \textbf{0.0133} & 54.75 && 4.09 \std{0.39}\\
        RLW & sgd & 0.05 &&         0.7070 & 0.9205 && 0.0176 & 123.13 && 48.84 \std{1.79} \\ \customdashline
        IMTL & adam & 0.001 &&   \textbf{0.7226} & \textbf{0.9259} && \textbf{\underline{0.0121}} & \textbf{45.25} && \textbf{-3.38} \std{0.92}\\ 
        IMTL & signSGD & 0.001  && 0.7177 & 0.9243 && 0.0128 & 49.61 && 0.57 \std{3.75}\\
        IMTL & sgd & 0.005 &&    0.7027 & 0.9192 && 0.0185 & 122.37 && 50.33 \std{3.30}\\ \customdashline
        PCGrad & adam & 0.001 && \textbf{\underline{0.7247}} & \textbf{\underline{0.9272}} && \textbf{0.0130} & \textbf{47.24} && \textbf{-0.58} \std{0.56}\\ 
        PCGrad & signSGD & 0.001  && 0.7187 & 0.9248 && 0.0132 & 53.35 && 3.28 \std{1.41}\\
        PCGrad & sgd & 0.05 &&   0.7083 & 0.9212 && 0.0173 & 122.52 && 47.90 \std{3.68}\\ \customdashline
        CAGrad & adam & 0.001 && \textbf{0.7245} & \textbf{0.9264} && \textbf{0.0124} & \textbf{45.56} && \textbf{-2.59} \std{0.68}\\ 
        CAGrad & signSGD & 0.001  && 0.7154 & 0.9243 && 0.0128 & 49.06 && 0.37 \std{0.41}\\
        CAGrad & sgd & 0.1 &&    0.7096 & 0.9220 && 0.0172 & 120.24 && 46.58 \std{2.21}\\ \customdashline
        AlignedMTL & adam & 0.0005 && \textbf{0.7225} & \textbf{0.9259} && \textbf{0.0122} & 47.70 && \textbf{-1.79} \std{0.70} \\ 
        AlignedMTL & signsgd & 0.001 && 0.7169 & 0.9241 && 0.0127 & \textbf{47.56} && -0.70 \std{0.61}
 \\
        AlignedMTL & sgd & 0.1 && 0.7096 & 0.9218 && 0.0174 & 120.38 && 46.94 \std{1.19}
 \\ \customdashline
        
        Adatask & adam & 0.001 && \textbf{0.7234} & \textbf{0.9260 } && \textbf{0.0124} &\textbf{47.21} && \textbf{--1.77} \std{0.86}\\
        MTL-IO & sgd & 0.05 && 0.7098 & 0.9217 && 0.0187 & 120.61 && 49.57  \std{2.28}\\
    \bottomrule
    \end{tabular}
\label{tab:res_cs_deeplab}
\end{table}


==> tables/res_cs_segnet.tex <==

\clearpage
\begin{table}[!ht]
    \centering
    \tiny
    % \setlength{\tabcolsep}{6pt}  % default: 6pt
    \newcommand{\gcs}{\hspace{12pt}}
    \newcommand{\customdashline}{\noalign{\vskip 0.5ex}\hdashline\noalign{\vskip 0.5ex}}
    \caption{
    \textbf{Results for different MTO methods and optimizers on Cityscapes\cite{cordts_cityscapes_2016} using SegNet~\cite{badrinarayanan_segnet_2017}.}
    The best score per metric is highlighted \textbf{for each MTO method} as well as \underline{over all methods and optimizers}.
    While different MTO methods perform best over the distinct metrics, models trained with Adam outperform those based on SGD+mom in most direct comparisons.
    On the overall $\Delta_m$ metric, Adam shows superior performance for all MTO methods, in some cases even with a high margin.
    Best performance for each metric was also achieved by using Adam.
    }
    \begin{tabular}{cccc@{\gcs}ccc@{\gcs}ccc@{\gcs}c}
    \toprule    
        &&&& \multicolumn{2}{c}{Sem.Seg.} && \multicolumn{2}{c}{Depth}\\
        \cmidrule(r){5-6} \cmidrule(r){8-9}
        MTO & Optimizer & lr && mIoU $\uparrow$ & pixAcc $\uparrow$  && AbsErr $\downarrow$  & RelErr $\downarrow$ && DeltaM $\downarrow$\\
    \midrule
        %STL & adam & && 0.7251 & 0.9290 && 0.0126 & 24.24 \\
        STL & adam & && 0.7122 & 0.9221 && 0.0134 & 29.88 \\
    \midrule
        EW & adam & 0.005 &&     0.6898 & 0.9165 && \textbf{0.0196} & \textbf{109.84} && \textbf{79.43} \std{3.68}\\ 
        EW & signSGD & 0.001  && \textbf{0.7013} & 0.9174 && 0.0210 & 115.67 && 86.52 \std{6.06}\\
        EW & sgd & 0.1 &&        0.6967 & \textbf{0.9179} && 0.0216 & 113.82 && 86.24 \std{1.97}\\ \customdashline
        UW & adam & 0.001 &&     \textbf{0.7052} & \textbf{0.9202} && \textbf{\underline{0.0136}} & \textbf{\underline{35.69}} && ~\textbf{\underline{5.44}} \std{2.38}\\ 
        UW & signSGD & 0.001  && 0.6506 & 0.8997 && 0.0166 & 53.61 && 28.54 \std{7.83}\\
        UW & sgd & 0.01 &&       0.6750 & 0.9110 && 0.0219 & 114.67 && 88.39 \std{1.35}\\ \customdashline
        RLW & adam & 0.001 &&    \textbf{0.7013} & \textbf{0.9196} && \textbf{0.0197} & \textbf{103.61} && \textbf{73.91} \std{7.63}\\ 
        RLW & signSGD & 0.0005  && 0.6962 & 0.9169 && 0.0204 & 112.46 && 82.90 \std{5.32}\\
        RLW & sgd & 0.1 &&       0.6918 & 0.9156 && 0.0227 & 113.59 && 88.16 \std{0.67}\\ \customdashline
        IMTL & adam & 0.005 &&   \textbf{0.6963} & \textbf{0.9170} && \textbf{0.0148} & \textbf{45.63} && \textbf{16.55} \std{1.52}\\ 
        IMTL & signSGD & 0.005  && 0.6659 & 0.9070 && 0.0197 & 101.90 && 74.03 \std{14.62}\\
        IMTL & sgd & 0.01 &&     0.6716 & 0.9107 && 0.0230 & 114.38 && 90.21 \std{0.74}\\ \customdashline
        PCGrad & adam & 0.01 &&  0.6770 & 0.9135 && 0.0226 & \textbf{103.88} && \textbf{80.56} \std{3.70}\\ 
        PCGrad & signSGD & 0.001  && 0.6929 & 0.9170 && \textbf{0.0210} & 113.32 && 84.74 \std{3.46}\\
        PCGrad & sgd & 0.1 &&    \textbf{0.6972} & \textbf{0.9176} && 0.0235 & 107.06 && 84.09 \std{0.93}\\ \customdashline
        CAGrad & adam & 0.001 && \textbf{0.7088} & \textbf{0.9208} && \textbf{0.0162} & \textbf{66.39} && \textbf{35.81} \std{14.91}\\ 
        CAGrad & signSGD & 0.001  && 0.6883 & 0.9138 && 0.0182 & 107.06 && 74.68 \std{18.91}\\
        CAGrad & sgd & 0.1 &&    0.6896 & 0.9156 && 0.0205 & 115.52 && 85.88 \std{0.31} \\ \customdashline
        AlignedMTL & adam & 0.0005 && \textbf{\underline{0.7164}} & \textbf{\underline{0.9246}} && \textbf{0.0154} & \textbf{64.89} && \textbf{32.76} \std{5.27}\\ 
        AlignedMTL & signSGD & 0.001 && 0.7010 & 0.9189 && 0.0180 & 102.41 && 69.77 \std{24.91} \\
        AlignedMTL & sgd & 0.1 && 0.6684 & 0.9103 && 0.0224 & 113.11 && 88.37 \std{0.53} \\ \customdashline
        Adatask & adam & 0.0005 && \textbf{0.7039} & \textbf{0.9196} && \textbf{0.0146} & \textbf{52.17} && \textbf{21.28} \std{0.35}\\ 
        MTL-IO & sgd & 0.1 &&    0.6957 & 0.9172 && 0.0233 & 110.19 && 86.46 \std{1.63} \\ 
    \bottomrule
    \end{tabular}
\label{tab:res_cs_segnet}
\end{table}

